Hot planets around cool stars -- two short-period mini-Neptunes transiting the late K-dwarf TOI-1260

We present the discovery and characterization of two sub-Neptunes in close orbits, as well as a tentative outer planet of a similar size, orbiting TOI-1260 - a low metallicity K6V dwarf star. Photometry from TESS yields radii of $R_{\rm b} = 2.33 \pm 0.10$ $R_{\oplus}$ and $R_{\rm c} = 2.82 \pm 0.15$ $R_{\oplus}$, and periods of 3.13 and 7.49 days for TOI-1260b and TOI-1260c, respectively. We combined the TESS data with a series of ground-based follow-up observations to characterize the planetary system. From HARPS-N high-precision radial velocities we obtain $M_{\rm b} = 8.61_{ - 1.46 } ^ { + 1.36 }$ $M_{\oplus}$ and $M_{\rm c} = 11.84_{ - 3.23 } ^ { + 3.38 }$ $M_{\oplus}$. The star is moderately active with a complex activity pattern, which necessitated the use of Gaussian process regression for both the light curve detrending and the radial velocity modelling, in the latter case guided by suitable activity indicators. We successfully disentangle the stellar-induced signal from the planetary signals, underlining the importance and usefulness of the Gaussian Process approach. We test the system's stability against atmospheric photoevaporation and find that the TOI-1260 planets are classic examples of the structure and composition ambiguity typical for the $2-3$ $R_{\oplus}$ range.

==> serval.tex <==
\begin{table*}
  \centering
  \caption{Radial velocities and spectral activity indicators measured from TNG/HARPS-N spectra.
    \label{serval}}
  \begin{tabular}{rrrrrrrrrrrrr}
    \hline
    \hline
%    \noalign{\smallskip}
    \multicolumn{1}{r}{BJD$_\mathrm{TBD}$} &
    \multicolumn{1}{r}{RV} &
    \multicolumn{1}{r}{$\sigma_\mathrm{RV}$} &
    \multicolumn{1}{r}{CRX} &
    \multicolumn{1}{r}{$\sigma_\mathrm{CRX}$} &
    \multicolumn{1}{r}{dlW} &
    \multicolumn{1}{r}{$\sigma_\mathrm{dlW}$} &
    \multicolumn{1}{r}{$\mathrm{H_{\alpha}}$} &
    \multicolumn{1}{r}{$\mathrm{\sigma_{H_{\alpha}}}$} &
    \multicolumn{1}{r}{$\mathrm{NaD_{1}}$} &
    \multicolumn{1}{r}{$\mathrm{\sigma_{NaD_{1}}}$} &
    \multicolumn{1}{r}{$\mathrm{NaD_{2}}$} &
    \multicolumn{1}{r}{$\mathrm{\sigma_{NaD_{2}}}$}\\ 
    \multicolumn{1}{r}{-2457000} &
    \multicolumn{1}{r}{($\mathrm{m\,s^{-1}}$)} &
    \multicolumn{1}{r}{($\mathrm{m\,s^{-1}}$)} &
    \multicolumn{1}{r}{($\mathrm{m\,s^{-1}\,Np^{-1}}$)} &
    \multicolumn{1}{r}{($\mathrm{m\,s^{-1}\,Np^{-1}}$)} &
    \multicolumn{1}{r}{($\mathrm{m^2\,s^{-2}}$)} &
    \multicolumn{1}{r}{($\mathrm{m^2\,s^{-2}}$)} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---}\\ 
%    \noalign{\smallskip}
    \hline
%    \noalign{\smallskip}
     1862.62923 &           6.677 &           1.716 &         -17.725 &          14.096 &          -2.805 &           3.196 &          0.6841 &          0.0020 &          0.2004 &          0.0024 &          0.2252 &          0.0026\\
     1862.66579 &           4.803 &           1.340 &          -9.964 &          11.112 &          -7.302 &           2.351 &          0.6850 &          0.0017 &          0.1974 &          0.0020 &          0.2216 &          0.0021\\
     1863.67080 &          10.163 &           1.235 &          10.432 &          10.103 &         -17.998 &           1.895 &          0.6832 &          0.0013 &          0.1945 &          0.0014 &          0.2200 &          0.0015\\
     1863.78184 &          11.454 &           1.180 &          10.563 &           9.470 &         -15.791 &           1.870 &          0.6844 &          0.0012 &          0.1951 &          0.0014 &          0.2196 &          0.0015\\
     1864.64888 &          15.901 &           1.490 &          14.765 &          12.360 &          -3.886 &           2.166 &          0.6855 &          0.0018 &          0.1975 &          0.0020 &          0.2236 &          0.0022\\
     1864.76150 &          13.179 &           1.573 &          20.240 &          13.193 &          -6.655 &           2.239 &          0.6827 &          0.0019 &          0.1968 &          0.0021 &          0.2284 &          0.0023\\
     1865.63156 &           5.489 &           1.193 &          14.321 &          10.311 &          -8.966 &           2.404 &          0.6816 &          0.0017 &          0.1991 &          0.0016 &          0.2245 &          0.0018\\
     1865.76718 &           1.903 &           1.434 &          19.806 &          11.892 &          -8.575 &           2.433 &          0.6913 &          0.0016 &          0.2000 &          0.0016 &          0.2219 &          0.0018\\
     1869.71163 &           0.562 &           1.555 &          -9.033 &          12.511 &          -1.288 &           2.907 &          0.6875 &          0.0017 &          0.2007 &          0.0021 &          0.2282 &          0.0023\\
     1896.56585 &          15.450 &           1.436 &          -3.060 &          11.637 &          -1.510 &           2.297 &          0.6878 &          0.0016 &          0.2237 &          0.0020 &          0.2459 &          0.0021\\
     1896.67552 &          13.918 &           1.388 &         -11.290 &          11.143 &          -0.808 &           2.814 &          0.6945 &          0.0016 &          0.2284 &          0.0020 &          0.2467 &          0.0022\\
     1898.56841 &           7.774 &           1.073 &          -3.532 &           8.928 &           0.857 &           2.620 &          0.7382 &          0.0014 &          0.2165 &          0.0015 &          0.2407 &          0.0016\\
     1925.63670 &          17.927 &           1.749 &          -2.160 &          14.638 &          -1.086 &           3.147 &          0.6863 &          0.0023 &          0.2479 &          0.0030 &          0.2599 &          0.0032\\
     1926.64886 &          19.622 &           2.118 &         -15.619 &          17.407 &           0.278 &           2.686 &          0.7005 &          0.0019 &          0.2343 &          0.0025 &          0.2600 &          0.0027\\
     1929.63674 &          10.128 &           1.193 &          -1.733 &          10.068 &          -7.456 &           2.374 &          0.6858 &          0.0018 &          0.2118 &          0.0020 &          0.2432 &          0.0022\\
     1930.42198 &          11.743 &           2.290 &         -24.218 &          19.108 &          -6.858 &           3.472 &          0.6937 &          0.0028 &          0.2339 &          0.0036 &          0.2459 &          0.0039\\
     1969.53394 &          -0.344 &           2.607 &          30.922 &          21.458 &         -23.205 &           3.971 &          0.6870 &          0.0031 &          0.3179 &          0.0047 &          0.3119 &          0.0049\\
     1971.52051 &          -2.375 &           1.298 &          -6.884 &          10.783 &         -44.328 &           2.698 &          0.6768 &          0.0016 &          0.2088 &          0.0019 &          0.2320 &          0.0021\\
     2000.41367 &           2.216 &           1.268 &          -8.945 &          10.158 &         -36.375 &           2.377 &          0.6827 &          0.0014 &          0.2021 &          0.0017 &          0.2323 &          0.0019\\
     2000.45426 &           4.378 &           1.489 &         -35.801 &          10.971 &         -25.136 &           2.493 &          0.6822 &          0.0015 &          0.2101 &          0.0021 &          0.2300 &          0.0022\\
     2001.42014 &           0.440 &           1.116 &         -11.500 &           8.915 &         -47.568 &           1.854 &          0.6692 &          0.0011 &          0.1937 &          0.0012 &          0.2238 &          0.0014\\
     2001.46039 &          -0.236 &           0.949 &         -23.011 &           7.095 &         -48.208 &           1.735 &          0.6705 &          0.0010 &          0.1916 &          0.0011 &          0.2242 &          0.0012\\
     2002.42024 &          -2.632 &           0.905 &           5.811 &           7.749 &         -53.132 &           2.055 &          0.6726 &          0.0014 &          0.1975 &          0.0014 &          0.2341 &          0.0016\\
     2002.46195 &          -0.506 &           1.311 &          13.103 &          10.881 &         -55.646 &           2.419 &          0.6712 &          0.0013 &          0.1967 &          0.0014 &          0.2353 &          0.0015\\
     2011.40922 &          27.029 &           2.205 &          -0.278 &          18.301 &         -29.220 &           3.238 &          0.6777 &          0.0024 &          0.1989 &          0.0033 &          0.2373 &          0.0036\\
     2011.44218 &          23.398 &           2.840 &          16.880 &          23.534 &         -32.558 &           4.204 &          0.6794 &          0.0034 &          0.2268 &          0.0054 &          0.2724 &          0.0060\\
     2012.40959 &          25.530 &           1.828 &          20.100 &          14.729 &         -24.200 &           2.180 &          0.6723 &          0.0016 &          0.2009 &          0.0020 &          0.2305 &          0.0022\\
     2012.44888 &          25.937 &           1.907 &          13.461 &          15.545 &         -27.838 &           2.505 &          0.6822 &          0.0018 &          0.2038 &          0.0022 &          0.2337 &          0.0024\\
     2013.42280 &          17.344 &           1.733 &          30.803 &          13.985 &         -20.223 &           2.502 &          0.6878 &          0.0020 &          0.2484 &          0.0025 &          0.2671 &          0.0026\\
     2013.44892 &          17.566 &           2.332 &           0.142 &          20.049 &         -13.318 &           4.085 &          0.6896 &          0.0035 &          0.2526 &          0.0049 &          0.2816 &          0.0054\\
     2013.47580 &          26.451 &           3.139 &          39.435 &          26.754 &          -9.109 &           5.318 &          0.6887 &          0.0042 &          0.3239 &          0.0064 &          0.3563 &          0.0069\\
     2014.42732 &          30.021 &           1.846 &          -7.137 &          15.000 &         -13.315 &           2.384 &          0.6837 &          0.0017 &          0.2265 &          0.0024 &          0.2527 &          0.0025\\
     2014.46531 &          28.500 &           1.704 &          16.641 &          13.691 &         -14.391 &           3.104 &          0.6796 &          0.0018 &          0.2181 &          0.0024 &          0.2506 &          0.0026\\
%    \noalign{\smallskip}
    \hline
  \end{tabular}
\end{table*}


==> table-rvs.tex <==
\begin{table*}
  \centering
  \caption{Radial velocities and spectral activity indicators measured from TNG/HARPS-N spectra for TOI-1260.
    \label{table-rvs}}
  \begin{tabular}{rrrrrrrrrrr}
    \hline
    \hline
%    \noalign{\smallskip}
    \multicolumn{1}{r}{BJD$_\mathrm{TBD}$} &
    \multicolumn{1}{r}{RV} &
    \multicolumn{1}{r}{$\sigma_\mathrm{RV}$} &
    \multicolumn{1}{r}{BIS} &
    \multicolumn{1}{r}{$\sigma_\mathrm{BIS}$} &
    \multicolumn{1}{r}{CCF\_FHWM} &
    \multicolumn{1}{r}{CCF\_CTR} &
    \multicolumn{1}{r}{S-index} &
    \multicolumn{1}{r}{$\sigma_\mathrm{S-index}$} &
    \multicolumn{1}{r}{SNR} &
    \multicolumn{1}{r}{$\mathrm{T_{exp}}$}\\
    \multicolumn{1}{r}{-2457000} &
    \multicolumn{1}{r}{(\mps)} &
    \multicolumn{1}{r}{(\mps)} &
    \multicolumn{1}{r}{(\mps)} &
    \multicolumn{1}{r}{(\mps)} &
    \multicolumn{1}{r}{(\kmps)} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{---} &
    \multicolumn{1}{r}{(s)}\\    
%    \noalign{\smallskip}
    \hline
%    \noalign{\smallskip}
    1862.62923 &           6.677 &           1.716 &          40.628 &           3.763 &           6.364 &          42.479 &           1.133 &           0.025 &            38.7 &          3600.0\\
    1862.66579 &           4.803 &           1.340 &          50.620 &           3.022 &           6.361 &          42.637 &           1.122 &           0.019 &            45.9 &          3600.0\\
    1863.67080 &          10.163 &           1.235 &          47.085 &           2.120 &           6.360 &          42.878 &           1.134 &           0.012 &            61.2 &          3600.0\\
    1863.78184 &          11.454 &           1.180 &          52.086 &           2.173 &           6.363 &          42.821 &           1.135 &           0.012 &            59.9 &          3600.0\\
    1864.64888 &          15.901 &           1.490 &          56.202 &           3.091 &           6.371 &          42.728 &           1.154 &           0.021 &            45.1 &          3600.0\\
    1864.76150 &          13.179 &           1.573 &          46.279 &           3.192 &           6.363 &          42.705 &           1.168 &           0.022 &            44.2 &          3600.0\\
    1865.63156 &           5.489 &           1.193 &          49.886 &           2.354 &           6.380 &          42.741 &           1.141 &           0.014 &            56.3 &          3600.0\\
    1865.76718 &           1.903 &           1.434 &          47.921 &           2.470 &           6.381 &          42.767 &           1.169 &           0.016 &            54.5 &          3600.0\\
    1869.71163 &           0.562 &           1.555 &          63.711 &           3.314 &           6.383 &          42.718 &           1.193 &           0.022 &            41.9 &          3600.0\\
    1896.56585 &          15.450 &           1.436 &          45.665 &           2.994 &           6.384 &          42.720 &           1.214 &           0.019 &            45.9 &          3600.0\\
    1896.67552 &          13.918 &           1.388 &          43.192 &           3.018 &           6.386 &          42.659 &           1.232 &           0.019 &            45.8 &          3600.0\\
    1898.56841 &           7.774 &           1.073 &          56.588 &           2.184 &           6.387 &          42.631 &           1.446 &           0.013 &            60.1 &          3600.0\\
    1925.63670 &          17.927 &           1.749 &          43.613 &           4.335 &           6.393 &          42.655 &           1.123 &           0.032 &            34.8 &          3600.0\\
    1926.64886 &          19.622 &           2.118 &          61.432 &           3.705 &           6.379 &          42.775 &           1.199 &           0.026 &            39.4 &          3300.0\\
    1929.63674 &          10.128 &           1.193 &          64.774 &           2.971 &           6.372 &          42.772 &           1.175 &           0.020 &            47.1 &          3006.7\\
    1930.42198 &          11.743 &           2.290 &          72.455 &           5.391 &           6.359 &          42.761 &           1.026 &           0.054 &            29.6 &          2200.0\\
    1969.53394 &          -0.344 &           2.607 &          52.253 &           6.453 &           6.339 &          42.808 &           1.146 &           0.041 &            25.9 &          3600.0\\
    1971.52051 &          -2.375 &           1.298 &          63.058 &           2.849 &           6.316 &          43.145 &           1.011 &           0.019 &            48.1 &          3600.0\\
    2000.41367 &           2.216 &           1.268 &          70.680 &           2.731 &           6.333 &          43.037 &           1.098 &           0.018 &            48.8 &          3600.0\\
    2000.45426 &           4.378 &           1.489 &          75.663 &           3.223 &           6.333 &          43.001 &           1.067 &           0.022 &            42.4 &          3600.0\\
    2001.42014 &           0.440 &           1.116 &          63.516 &           1.940 &           6.312 &          43.220 &           1.038 &           0.010 &            65.8 &          3600.0\\
    2001.46039 &          -0.236 &           0.949 &          73.278 &           1.702 &           6.312 &          43.235 &           1.024 &           0.009 &            73.8 &          3600.0\\
    2002.42024 &          -2.632 &           0.905 &          56.605 &           1.996 &           6.303 &          43.312 &           1.001 &           0.011 &            64.2 &          3600.0\\
    2002.46195 &          -0.506 &           1.311 &          63.482 &           1.999 &           6.302 &          43.323 &           1.024 &           0.011 &            64.4 &          3600.0\\
    2011.40922 &          27.029 &           2.205 &          48.672 &           5.219 &           6.321 &          43.031 &           1.123 &           0.041 &            30.2 &          3300.0\\
    2011.44218 &          23.398 &           2.840 &          54.360 &           8.605 &           6.334 &          42.874 &           1.069 &           0.075 &            20.8 &          2999.1\\
    2012.40959 &          25.530 &           1.828 &          33.998 &           3.095 &           6.349 &          42.922 &           1.105 &           0.021 &            45.2 &          3300.0\\
    2012.44888 &          25.937 &           1.907 &          45.139 &           3.518 &           6.342 &          42.933 &           1.157 &           0.026 &            40.7 &          3300.0\\
    2013.42280 &          17.344 &           1.733 &          35.178 &           3.499 &           6.354 &          42.858 &           1.152 &           0.024 &            41.5 &          3300.0\\
    2013.44892 &          17.566 &           2.332 &          54.908 &           7.476 &           6.371 &          42.777 &           1.121 &           0.063 &            23.7 &          1353.0\\
    2013.47580 &          26.451 &           3.139 &          14.612 &           8.586 &           6.351 &          42.772 &           1.103 &           0.075 &            21.0 &          2273.7\\
    2014.42732 &          30.021 &           1.846 &          46.902 &           3.644 &           6.370 &          42.766 &           1.168 &           0.027 &            39.5 &          3300.0\\
    2014.46531 &          28.500 &           1.704 &          39.564 &           3.733 &           6.360 &          42.848 &           1.165 &           0.029 &            39.0 &          3300.0\\
%    \noalign{\smallskip}
    \hline
  \end{tabular}
\end{table*}

